Design of an Adaptive Lightweight LiDAR to Decouple Robot-Camera Geometry

A fundamental challenge in robot perception is the coupling of the sensor pose and robot pose. This has led to research in active vision where robot pose is changed to reorient the sensor to areas of interest for perception. Further, egomotion such as jitter, and external effects such as wind and others affect perception requiring additional effort in software such as image stabilization. This effect is particularly pronounced in micro-air vehicles and micro-robots who typically are lighter and subject to larger jitter but do not have the computational capability to perform stabilization in real-time. We present a novel microelectromechanical (MEMS) mirror LiDAR system to change the field of view of the LiDAR independent of the robot motion. Our design has the potential for use on small, low-power systems where the expensive components of the LiDAR can be placed external to the small robot. We show the utility of our approach in simulation and on prototype hardware mounted on a UAV. We believe that this LiDAR and its compact movable scanning design provide mechanisms to decouple robot and sensor geometry allowing us to simplify robot perception. We also demonstrate examples of motion compensation using IMU and external odometry feedback in hardware.

==> intro-old.tex <==
\section{Introduction}
Modern autonomy is largely driven by vision and depth sensors for perception. Most such techniques make an implicit assumption that the relative pose of the sensor w.r.t. the robot is fixed, and changes in sensor viewpoint require a change in the robot pose. This means that fast moving robots must deal with motion compensation (i.e. camera-robot \emph{stabilization}). Correspondingly, this is a widely studied problem in robotics and vision ~\cite{neuhaus2018mc2slam,gojcic2019perfect,taketomi2017visual,phelps2019blind}.

While successful, most such methods compensate through \emph{post-capture} processing of sensor data. We contend that this is simply not feasible for the next generation of fast miniature robots such as robotic bees \cite{robobees-sciam13}, crawling and walking robots \cite{hoffman2013design}, and small UAVs (unmanned aerial vehicle) \cite{mulgaonkar2015design}. Without proper motion compensation for these devices, we will not be able to unlock the full potential of what is one of the ten grand challenges in science robotics~\cite{yang2018grand}. 

This paper shows the motion compensation advantage of decoupling robot-camera geometry, and providing the ability to control the camera properties independent of the robot pose could bring about a new perspective to robot perception and simplify the autonomy pipeline.

\section{Key Idea: Motion Compensation \emph{in} Hardware}
\kar{the first two paragraphs here are somewhat redundant to the intro}

The egomotion of small robots (and onboard sensors) is quite extreme making any sensing challenging. For example, flapping-wing robots such as the RoboBee exhibit a high frequency rocking motion (at about 120 Hz) due to the piezo-electric actuation \cite{helbling2014pitch}. Environmental factors such as wind affect micro-robots to a greater extent than a larger robot. There might be aerodynamic instability due ornithopter-based shock absorption \cite{xue2019computational}. 

While there have been software methods to correct for such effects for cameras \cite{chen2009real} and LiDARs \cite{peng2007model}, this is often difficult to perform in real-time onboard due to the computational, energy  and latency constraints on the robot mentioned above. It would be ideal for sensors to perform such correction in hardware without requiring onboard computing help. In this work, we propose the design of an IMU-compensated LiDAR to address this challenge. 

Most systems today leave the difficult problem of motion estimation and compensation to post-capture algorithms such as optical flow-based registration. In contrast, animal eyes have fast mechanical movements that compensate for motion, in real-time and at high accuracy \cite{alldieck2017optical}. In Figure \ref{fig:hawk}, we show frames $V(t)$ from a video of a hawk (\emph{Buteo jamaicensis}) being moved by a human trainer \cite{youtube_2020}. We also show the average of the video $\sum_t \frac{V(t)}{T}$ over a time interval T. Note that the averaged image shows motion blurring, except where the eagle mechanically compensates for the shifts. 


\begin{figure}
  \centering
  \includegraphics[width=0.9\linewidth]{hawk.jpg}
  \caption{Biological motion compensation. 
  \href{https://www.youtube.com/watch?v=aqgewVCC0k0}{https://www.youtube.com/watch?v=aqgewVCC0k0}}
  \label{fig:hawk}
\end{figure}

% These capabilities are compelling to humans -- this video has been seen over 50k times on Youtube, and many such demonstrations exist for animals such as chickens (> 4M views) and owls (> 40k views). We encourage the reader to view some of these to understand the capabilities . 

We envision biologically-inspired motion compensation that happens during sensing. These sensors need to adaptively change their orientation, in real-time, and in concert with robot goals such as mapping or navigation. Effectively, the rotation matrix R must cancel out robot motion. 

For the first time, we use a custom designed microelectromechanical (MEMS) mirror with a real-time inertial measurement unit inside a simple yet effective system-level sensor design for a light ranging (LIDAR) device. The LIDAR is designed such that its heavy and power-hungry components are separated, so that the lightweight components can fit on micro-air vehicle flight payloads. We then demonstrate our motion compensated LIDAR with an autonomous UAV, showing for the first time ever, biologically inspired motion compensation on a robot in real-time. 

\section{Theoretical Strategy: Decoupling Robot-Camera Geometry}

Our key idea is to build a sensor design that can decouple robot-camera geometry, and provide the ability to control the camera properties independent of the robot pose. Such sensors could bring about a new perspective to robot perception and simplify the autonomy pipeline. We contend that this decoupling will propel a paradigm shift for robotic perception, particularly in underactuated robots. 

Such a breakthrough has been the goal of previous efforts, collectively termed as active vision \cite{paul2021camtuner} --- however, active vision in robotics has not reached its full potential, partly because of its dependence on PTZ (point-tilt-zoom) cameras and similar technologies that use mechanical actuation. In fact, most robots do not have PTZ-like technology and cameras are usually simply rigidly attached to robots. Therefore, robotics today is constrained within the degenerate case of active vision, where robot pose determines camera pose.

In this paper, we show new sensor designs for decoupling this robot-dominated relative robot-camera pose and demonstrate that, even over small time periods, these designs can enable novel applications for robot perception. 

\subsection{Motivation for Decoupling}

To see why decoupling is useful, we start with the well-understood form of camera-robot geometry.  If the robot is at the origin, then the camera pose is given by the rotation and translation matrices $[R_c t_c]$, and the image pixels are related to this pose change by sensor parameters $K$, containing properties such as focal length and pixel pitch. 

Let us consider a perception task such as Visual SLAM. As the robot is traversing the environment, its motion causes a change in the camera pose allowing the camera to see new parts of the scene. These are then processed into a map of the environment and localize the robot in that map. If there is no decoupling, then the camera experiences all the motion the robot experiences, including jitter and other potential disturbances that are detrimental to the Visual SLAM task. Further, if the system also needs to track targets, the robot pose changes for navigation may not coincide with the optical camera pose for tracking. The ability to decouple the poses and control the camera pose allows us to alleviate such motion allowing the camera to better perform the robot perception task. 

\subsection{Uncoupling within Brief Intervals}
\kar{better section heading?}

This work demonstrates camera designs that break through these past difficulties, by exploiting recently available microelectromechanical (MEMS) and opto-mechanical components for changing camera parameters. Opto-MEMS components are famously fast (many KHz), and they allow the changing of the camera projection matrix $P = K[R_c t_c]$ during robot motion, such that the robot is effectively static. By changing camera views two orders of magnitude (or more) faster than robot motion, we can effectively decouple the two allowing for camera views independent of the robot view. Such a decoupling allows the robot to focus on the control task while the camera can perform perception (which is required for the control task) independently. This decoupling greatly simplifies robot planning as the planner does not need to account for perception and just needs to reason about the control task at hand.  

%\subsection{Impact}

%Our framework can enable high-end imaging applications on robots as they move through difficult environments, on agile platforms, or in conditions with sparse features. Our contributions are:

%\begin{enumerate}

%\item High-performance motion compensation and image stabilization: This is the focus of the current paper, where the rotation matrix Rc is adaptively controlled such that the camera is independent of robot jitter and shake.

%\item Distributed sensor attention and resolution control: In \cite{tasneem2020adaptive}, the author controlled the focus (diagonal in K) and distributed LIDAR resolution around a robot. With multiple robots, it is possible to have multiple, zooming cameras at a single target, across multiple moving robotic platforms.

%\item Controlled motion deblurring: Controlled motion blurring, such as parabolic motion \cite{choi2011motion}, has been known to improve image recovery, and these can be implemented during motion capture on robotic platforms.

%\item Synthetic aperture imaging across robots: Recent work in Science Robotics \cite{schedl2021autonomous} has shown that confocal imaging from drones can ‘see through’ foliage, and these types of synthetic aperture imaging. Expanding this to multiple robots would increase the aperture even further, and our approach can help with this. 

%\item Efficient EKF(extended kalman filter) SLAM: If our approach is *not* used, then the relative camera-robot pose ambiguity is yet another unknown variable that must be estimated by an EKF-enabled SLAM algorithm. Instead, by uncoupling these, we reduce the unknowns, enabling faster convergence for EKF SLAM and related methods. 

%\end{enumerate}

%In this paper, and in the next section, we focus particularly on the first of these applications; high-performance motion compensation and stabilization, since it is a turnkey technology on which every other application must be built upon. 

\kar{are there PDF versions of these images? }

\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{scan.png}
    %\includegraphics[width=.22\linewidth,trim={0 20pt 0 20},clip]{dim.PNG}
    %\includegraphics[width=.22\linewidth,trim={20pt 0 20 0},clip]{int.PNG}
    \includegraphics[width=0.2\textwidth]{dim.PNG}
    \includegraphics[width=0.2\textwidth]{int.PNG}
    %\includegraphics[width=.25\linewidth,trim={0 20pt 0 20},clip]{figures/robobee.PNG}
    %\includegraphics[width=.25\linewidth,trim={20pt 0 20 0},clip]{figures/walker.PNG}
    %\includegraphics[width=.32\linewidth,trim={70pt 0 50 20},clip]{figures/crazyflie.PNG}
    % \includegraphics[width=.25\linewidth,trim={70pt 0 50 20},clip]{figures/crazyflie.PNG}
    \caption{Our design is given above with the prototype motion-compensated LiDAR (up), and we also prepared a design for future work to integrate this onto smaller platforms.}
    \label{fig:futuristic}
    \vspace{-10pt}
\end{figure}

\subsection{Our Contribution: MEMS-based Decoupling for LIDAR}

Microelectromechanical (MEMS) technology provides a viable alternative for laser scanner that can minimize the weight and size of the LiDAR \cite{tasneem2020adaptive, kasturi2016uav, kimoto2014development}. However, even with the MEMS mirror's small size and light weight, the LiDAR is still too large and heavy because of other necessary components, like the laser, photodetector, optics, the driver circuit, and the signal processing circuitry. Furthermore, to enable real-time compensated scanning, the MEMS mirror direction must be controlled for arbitrary orientations in real-time. 
We solve the twin challenges of form-factor and egomotion with the following algorithmic and design contributions:


%Microelectromechanical (MEMS) technology provides a viable alternative for laser scanner that can minimize the weight and size of the LiDAR \cite{tasneem2020adaptive, kasturi2016uav, kimoto2014development}. However, even with the MEMS mirror's small size and light weight, the LiDAR is still too large and heavy because of other necessary components, like the laser, photodetector, optics, the driver circuit, and the signal processing circuitry. Furthermore, to enable real-time compensated scanning, the MEMS mirror direction must be controlled for arbitrary orientations in real-time. 

%Comparing to motorized image stabilization system \cite{jia2017system}, MEMS mirrors not only have the advantages of smaller size and light weight, the frequency response bandwidth of the MEMS mirrors are better than the bulky and heavy camera stabilizer. This would contribute to faster compensation response for high frequency motion jitter on microrobotics \cite{wang2017ultra, milanovic2017closed, filhol2005resonant}.  


%we have created a new LiDAR design and accompanying algorithms. Our contributions in this work are:

\begin{itemize}
    \item We present a simple, effective design, Figure~\ref{fig:futuristic}, where the LiDAR power and laser are delivered by tethers. Only the tether tip, the MEMS mirror, and photodetector will move with the micro-robot. 
    
    \item We adopted an electrothermal MEMS mirror similar to LiDAR scanner \cite{wang2020low}. This design enables wide non-resonant scanning angle for arbitrary orientations. 
    % It has a fast response time (5 ms), allowing high frequency egomotion compensation (up to 200 Hz).  Experiment does not support 200Hz compensation
    
    \item We show a proof-of-concept prototype combining an inertial measurement unit (IMU) with the MEMS mirror for egomotion compensation. The frequencies of the mirror modulation and IMU measurement are much higher than typical robot egomotion challenges. Our prototype IMU-based MEMS compensated scan system can perform such compensation in under 10 ms. 
    
    \item We describe and geometrically characterize our sensor, showing that compensation in hardware can reduce the number of unknowns for proprioceptive and exteroceptive tasks such as Simultaneous Localization and Mapping (SLAM). In simulation, we characterize the effect of compensation delay and compensation rate to identify benefits for sensing on micro-robots. 
\end{itemize}

Our envisioned design for the use of such a LiDAR as well as an image of our prototype are shown in Figure \ref{fig:futuristic}. 




%The futuristic design of the LiDAR for a microrobotics is shown in Figure \ref{fig:futuristic}. Figure \ref{fig:digaram} shows the schematic of the motion compensated LiDAR with a movable LiDAR head. 

%We propose a sensing system that shares in the computational burden, dividing the task of jitter compensation more equitably between sensor measurements and software, reducing both computational load and latency. We achieve this by compensating for the jitter in the LIDAR measurements by using a fast, light-weight MEMS mirror augmented with an IMU system. Both the MEMS mirror modulation capacity and the IMU frequency are much higher than the types of jitter we normally face for microrobotic systems. %We show that a conventional combination of Kalman filter and 3D SLAM, that obtains measurements from such a sensor, has fewer unknowns to estimate and therefore takes fewer iterations to converge. 

